CaliScalpel: In-Situ and Fine-Grained Qubit Calibration Integrated with Surface Code Quantum Error Correction

Quantum Error Correction (QEC) is a cornerstone of fault-tolerant, large-scale quantum computing. However, qubit error drift significantly degrades QEC performance over time, necessitating periodic calibration. Traditional calibration methods disrupt quantum states, requiring system downtime and making in situ calibration infeasible. We present CaliScalpel, an innovative framework for in situ calibration in surface codes. The core idea behind CaliScalpel is leveraging code deformation to isolate qubits undergoing calibration from logical patches. This allows calibration to proceed concurrently with computation, while code enlargement maintains error correction capabilities with minimal qubit overhead. Additionally, CaliScalpel incorporates optimized calibration schedules derived from detailed device characterization, effectively minimizing physical error rates. Our results show that CaliScalpel achieves concurrent calibration and computation with modest qubit overhead and negligible execution time impact, marking a significant step toward practical in situ calibration in surface-code-based quantum computing systems.

==> TexFile/02_introduction_01.tex <==
\section{Introduction}
\label{sec: introduction}

% Quantum Error Correction is steadily becoming a reality, with popular codes such as the surface code being validated across various hardware platforms. It seems that if we can build more high-quality qubits, we can potentially run programs that are fully protected by QEC. Ideally, we could select an appropriate code distance based on the size of the program, ensuring the desired level of protection for a given quantum computation. For instance, programs running on superconducting qubits could maintain a reasonable runtime probability under these conditions.

Quantum Error Correction (QEC) is essential for realizing large-scale fault-tolerant quantum computing and remains the only viable path forward \cite{gottesman1998theory, shor1996fault, lidar2013quantum}. Recent breakthroughs in QEC have demonstrated its feasibility, with significant progress achieved over the past few years \cite{acharya2024quantumerrorcorrectionsurface, google2021exponential, Bluvstein2024}. Notably, experiments such as Google's demonstration of a surface code operating below the error threshold have provided compelling evidence that QEC can effectively suppress logical errors \cite{}. 
%
These advancements highlight the potential of QEC to enable practical, fault-tolerant quantum programs.


% Unfortunately, maintaining an ideal logical error rate over the anticipated runtime of a program is highly challenging without frequent calibration. 
% Data analysis shows that without regular calibration, qubit gate errors increase rapidly. Our collected data illustrates this issue, with both small- and large-scale plots showing a steep rise in error rates over time without intervention.

However, running large-scale quantum computations in a fault-tolerant manner remains fraught with challenges, particularly when considering the long runtimes involved. For realistic applications~\cite{Gidney2021howtofactorbit, femoco}, computations may extend over hours or even days, during which qubit parameters can drift significantly, resulting in a substantial increase in error rates. Maintaining a consistent logical error rate over these extended periods becomes nearly impossible without frequent calibration.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/error_drift.png}
    \caption{Noise drift with in short-term and long-term.}
    \label{fig: error drift and calibration}
\end{figure}


\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/overview.png}
    \caption{
    Motivation example
    }
    %Deformation framework for excluding the defective qubits while maximally preserving the error resilience of the remaining function qubits. (b) Enlarge the code to restore the QEC capability. (c) Qubit layout design with an additional inter-space of $\Delta d$ saved for potential code expansion, facilitating qubit communication. \todoFX{Revise}
   %An example of implementing a CNOT gate involving an enlarged logical qubit is presented. Within this qubit layout, the enlarging directions of defective logical qubits are scheduled according to the location of defects and the on-going computational tasks (bottom-right part).
    \label{fig: introduction}
\end{figure*}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.47\textwidth]{Figures/motivation.png}
\label{fig: motivation}
\caption{motivation example}
\end{figure}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Figures/Main_table.png}
% \end{figure*}

% Our work aims to address the critical challenge of integrating Quantum Error Correction (QEC) with calibration. We analyzed existing methods for managing error drift and identified several approaches:

% (1) Passive Handling: This approach anticipates drift errors without performing real-time calibration, instead adjusting the final code distance to account for accumulated errors. However, preliminary calculations reveal that this method is ineffective, especially for longer runtimes. The data suggests that errors will likely exceed the threshold well before the program completes, rendering this method impractical.

% (2) Stalling: In this method, the entire program is paused, the logical qubits are moved to a calibrated space, and the quantum processing unit (QPU) is recalibrated. However, this leads to significant time and qubit overhead due to the migration and stalling of the entire program.

% (3) Statistical Method: The approach presented in~\cite{kelly2016scalable} uses detection events—specifically the rate at which errors occur—as a metric to inform control parameters, eliminating the need to interrupt error detection for calibration. However, it is suboptimal for two key reasons: 1. Control parameters must be inferred from the error syndrome, introducing inaccuracies. 2. The degeneration issue in QEC codes means different errors can produce the same syndrome. While this is not a problem for QEC (since the correction operation remains the same due to this degeneration), it complicates identifying which qubit is faulty, making it difficult to obtain reliable detection events from the QEC syndrome.

Addressing error drift in quantum computing using simple, heuristic approaches proves inadequate for large-scale, long-duration quantum programs. One such approach, which we term passive handling, involves preemptively adjusting the code distance based on projected error accumulation, while foregoing real-time calibration. Although this approach might appear viable, our analysis indicates that it fails for extended runtimes, as error accumulation quickly reaches unacceptable levels, compromising program completion. Another intuitive method, which we call stalling, involves pausing the quantum program to recalibrate the quantum processing unit (QPU). While this can improve gate fidelity, it introduces significant overhead due to the need to move logical qubits and halt the entire computation, resulting in excessive time and resource costs.

\YS{These naive approaches highlight the inherent challenges of maintaining error correction without real-time calibration. The only way to ensure consistent error suppression over long runtimes is to integrate calibration directly into the QEC process, allowing for continuous adjustment of control parameters in response to error drift. However, performing calibration concurrently with QEC presents significant challenges, particularly due to the need to maintain logical qubit coherence without disrupting the error correction cycle. This necessitates a sophisticated strategy to synchronize calibration with QEC operations, ensuring that both processes can run in tandem without compromising the logical state of the quantum computation. The critical question becomes: \textbf{How can we achieve efficient calibration during runtime while preserving the integrity of the QEC cycle?}}

\YS{To address this question, preliminary approaches have been explored, aiming to enable calibration without compromising the QEC process. One such approach, described in [4], attempts to calibrate based on detection events. This statistical approach updates control parameters using error rates inferred from error syndromes without interrupting error detection. However, this method faces significant limitations: inaccuracies in inferring control parameters from syndromes and complications arising from the degeneracy of QEC codes. Degeneracy—where different physical errors produce identical error syndromes—makes it difficult to accurately identify the faulty qubit, thereby reducing the effectiveness of this approach.}

We believe that the best solution lies in having QEC and calibration run in tandem. This raises important questions around timescales: How long does calibration take? How does it interact with the QEC cycle? Since QEC requires continuous operation to preserve logical states, it cannot simply be paused for calibration. The challenge, then, is how to balance these two processes.

This brings us to our proposed solution. Current calibration approaches do not fully account for the heterogeneous quality of individual qubits. In this paper, we propose a hardware-aware fine-grained calibration method that isolates specific gates and qubits using code deformation techniques from the surface code. By selectively performing destructive calibration on lower-quality qubits and gates, we can enhance overall efficiency without significantly affecting the logical error rate.




==> TexFile/02_introduction_lastnight.tex <==
\section{Introduction}
\label{sec: introduction}

% Quantum Error Correction is steadily becoming a reality, with popular codes such as the surface code being validated across various hardware platforms. It seems that if we can build more high-quality qubits, we can potentially run programs that are fully protected by QEC. Ideally, we could select an appropriate code distance based on the size of the program, ensuring the desired level of protection for a given quantum computation. For instance, programs running on superconducting qubits could maintain a reasonable runtime probability under these conditions.

Quantum Error Correction (QEC)~\cite{nielsen2010quantum, gottesman1998theory, shor1996fault, lidar2013quantum} is essential to enable large-scale Fault-Tolerant Quantum Computing (FTQC)  suitable for practical applications~\cite{shor1999polynomial, cao2019quantum}. Among various QEC schemes, %\cite{calderbank1996good, steane1996multiple, bombin2006topological, kitaev2003fault, fowler2012surface}
\emph{surface codes}~\cite{bravyi1998quantum, dennis2002topological, litinski2019game, beverland2022surface, fowler2012surface} have emerged as the leading solution and have been successfully implemented on various quantum hardware~\cite{acharya2024quantumerrorcorrectionsurface, google2023suppressing, zhao2022realization, Bluvstein2024}. Surface codes work by encoding \emph{logical qubits} into redundant physical qubits arranged in a 2D square or hexagonal lattice, effectively reducing the error rate of the logical qubits if the physical error rate remains below a certain \emph{threshold}~\cite{fowler2012surface}. With increasing code size, surface codes provide exponential suppression of logical errors. Recent experiments on superconducting devices~\cite{huang2020superconducting, bravyi2022future} demonstrated this error suppression for the first time~\cite{acharya2024quantumerrorcorrectionsurface}, underscoring the practical applicability of surface codes. 
%viability and scalability


% Unfortunately, maintaining an ideal logical error rate over the anticipated runtime of a program is highly challenging without frequent calibration. 
% Data analysis shows that without regular calibration, qubit gate errors increase rapidly. Our collected data illustrates this issue, with both small- and large-scale plots showing a steep rise in error rates over time without intervention.
% Despite the demonstrated effectiveness of surface codes, variations in hardware conditions significantly limit its performance.
% \YS{this sounds like QEC designer didn't consider hardware variations, also, the problem is not entirely about variations, but just about noise-level itself. Should be sth about QEC codes have their best working range and has its limitations about noise types (for example coherent errors) and noise levels. Especially, QEC cost is very very sensitive to noise-level (see fig.4 in~\cite{SurfaceCode}).} 

Despite their demonstrated effectiveness, surface codes are highly sensitive to noise levels — small increases in physical error rates can require substantial expansion in code size to maintain the same logical error rate~\cite{SurfaceCode}. Consequently, maintaining a low and stable physical error rate is essential to ensure the effectiveness of surface codes during long computations. 
%\YS{(Then, we switch over to error drifts in a new paragraph---) 
However, achieving such stability is challenging due to temporal variations in physical error rates in current quantum processors. Qubit and gate conditions degrade over time, leading to increased physical error rates—a phenomenon known as \emph{error drift}~\cite{proctor2020detecting, zhang2020error}. % Unfortunately, QEC becomes ineffective when error rates exceed certain threshold values~\cite{gottesman2010introduction, shor1996fault, aharonov1997fault, fowler2012surface, preskill1998reliable}, failing to maintain the expected robustness of the quantum system. \YS{this sentence should be moved to earlier or removed, also, threshold, physical error rate, logical error rate,  all need definitions in the intro} 
Fig.~\ref{fig: error drift and calibration}(a) illustrates the error drift observed on 
%Rensselaer
an IBM quantum computer~\cite{edman2024hardware}, showing that after just one day, over 90\% of single qubit gates exhibit error rates exceeding the threshold of surface codes. Theoretical estimates suggest that practical quantum applications are expected to run for hours or even days~\cite{Gidney2021howtofactorbit, femoco, litinski2023compute, babbush2018encoding}, assuming a fixed error rate. However, in practice, error drift can significantly undermine computational reliability, making such long computations infeasible.
%unaddressed 

\begin{figure}[t]
\vspace*{0.1cm}
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/error_drift.pdf} \\
    \hspace*{0.5cm} (a)  \hspace*{3.8cm} (b)    \vspace*{-0.3cm} \\
    \caption{Error drift on an IBM quantum computer: (a) Calibration maintains low physical error rates. (b) Without calibration, a majority of qubits exceed the surface code threshold after 24 hours.}
    \label{fig: error drift and calibration}
\vspace*{-0.5cm}
\end{figure}

\emph{Calibration}~\cite{kelly2018physical, klimov2020snake, tornow2022minimum, wittler2021integrated, tannu2019not} is the process of fine-tuning quantum hardware to maintain low physical error rates and counteract error drift. Quantum hardware installations frequently calibrate their devices-often several times a day-to keep qubits and gates aligned with optimal conditions. %\YS{Here, add a sentence to give an anecdote about how many times hardware providers like IBM calibrate in a day.} 
Calibration involves three key steps: characterization, control parameter adjustment, and validation. Importantly, the calibration process disrupts quantum states, making qubits under calibration unavailable for computation. 

The fundamental challenge in surface code based quantum computation lies at the intersection of two competing requirements: maintaining consistently low physical error rates (through calibration) while simultaneously preserving quantum information for ongoing computation. This tension motivates our central research question: {\it How can we integrate runtime calibration with ongoing computation at the program level while maintaining the reliability of surface code protected quantum programs?}


%\YS{This sentence aims to give a intuitive explanation to what does calibration does, but "verifying system performance" is way too abstract.} 



% Therefore, developing an approach that integrates calibration with the computation process is challenging but essential for preserving QEC functionality and ensuring the reliability of long-running programs.\YS{This sentence is the climax. Take better care of writing it.} 

% \YS{Calibration is not a technique}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\textwidth]{Figures/IntroOverview.pdf}
    \caption{Comparison of~\frameworkName~and  \baseline. (a) Error drift pattern in physical qubits. (b) Increased code distance approach. (c)~\baseline, a coarse-grained approach with high overhead. (d)~\frameworkName~enables \textit{in situ} calibration.}
    \vspace*{-0.3cm}
    \label{fig: introduction}
\end{figure*}


% A natural starting point draws inspiration from classical operating systems' management of concurrent memory access~\cite{computer_arch_book}. Just as classical processes compete for memory access, calibration and logical computation can be viewed as separate processes vying for the same qubit resources. 
% \dean{I don't love this analogy.  Better, I think, would be memory access vs refresh, or memory access vs. concurrent garbage collection.  But also would be okay with no analogy, as the concept
% is not a difficult one.}

A natural starting point draws inspiration from classical computing systems, where memory access must be coordinated with periodic DRAM refresh cycles [28]. Just as memory refresh temporarily interrupts access to maintain data integrity, qubit calibration requires periodic access to physical qubits while trying to preserve quantum information. 

However, key differences exist between the classical and quantum settings. While classical memory can be refreshed at the bit level, quantum error correction creates a critical constraint: individual physical qubits cannot be naively removed for calibration without catastrophic error propagation. Simply mirroring classical strategies leads to a conservative approach,  which we term \emph{\baselineLong} (\baseline): transferring entire logical qubits to ancillary regions via logical SWAP operations before calibrating their physical components~(\cref{fig: introduction}c). This classically inspired approach suffers from two fundamental limitations. First, 
 unlike classical bit copying, quantum logical SWAP operations require complex sequences of physical operations or quantum teleportation protocols~\cite{litinski2019game, beverland2022surface}, introducing substantial overhead in both ancilla qubit count and execution time. Second, there is a critical granularity mismatch—calibration operates at the physical qubit level, while computation occurs at the logical qubit level. Since physical qubits drift at varying rates~(\cref{fig: error drift and calibration}b),~\baseline~inefficiently forces entire logical qubits to pause when only a single physical qubit requires calibration, leading to high overheads that scale with worst-case behavior.

\begin{comment}


 These observations highlight two key requirements for practical calibration integration during runtime:
\begin{itemize}
    \item Physical-level qubit separation to reduce the frequency of calibration.
    \item {\it In situ} calibration to avoid costly logical SWAP operations.    
\end{itemize}


    At a high level, these limitations stem from the inherent conflict between calibration and computation processes: calibration requires disrupting quantum states, while computation seeks to preserve and manipulate them as desired. \YS{repetitive with earlier paragraphs} Consequently, achieving concurrency between these processes comes at a cost—significant space-time overhead in \policyTwoName~approach. \YS{Not insightful enough. Didn't actually explain the cost on a high-level.} Nevertheless, we still ask: \emph{Is it possible to achieve efficient calibration during runtime while enabling continuous computation protected by QEC?} \YS{I think this question should be asked before any solutions are proposed.}

\YS{What's our insight? Informally: the granularity of calibration is on the physical qubit level. And the quantum information in surface code is collectively encoded in a logical patch. This redundancy in the collective logical state allows us to decouple the physical qubit under calibration from logical computation without losing quantum information. There are existing tools for achieving it--- code deformation. }
\end{comment}


To overcome these limitations, we  propose\textbf{~\frameworkName}, a novel QEC framework that enables seamless integration of runtime calibration  with surface code protected quantum computation (\cref{fig: introduction}d).~\frameworkName's design builds on a key insight: {\it while naively removing physical qubits for calibration would catastrophically compromise error correction, surface codes permit strategic runtime update of their code structures to create calibration regions while preserving both logical information and error protection}.  

Building on this insight, ~\frameworkName~employs {\it code deformation}~\cite{yin2024surf, vuillot2019code, bombin2009quantum}, a technique that enables fine-grained runtime modification of the surface code structure while preserving logical information.~\frameworkName~designs and formalizes novel code deformation instruction sets for both square and hexagonal surface codes. The instruction sets enable two complementary operations: \emph{selective qubit isolation} creates temporary boundaries to separate physical qubits for calibration, while \emph{dynamic code enlargement} slightly enlarges affected patches to maintain error correction capabilities throughout the calibration process. 

\frameworkName~combines this instruction set with intelligent scheduling to create an efficient, automated calibration system. This system encompasses preparation time device characterization, compilation time calibration generation, and runtime calibration execution.  

During preparation,~\frameworkName~characterizes the device, capturing three key metrics for calibration optimization: calibration time, drift rate, and calibration crosstalk. At compilation time,~\frameworkName~analyzes this data to generate highly optimized calibration schedules that balance multiple competing objectives, including error rates, calibration frequency, and resource utilization. At runtime, QECali executes the pre-computed schedules using the defined instructions to isolate qubits and enlarge logical qubit patches.  
% \dean{you say "optimal" here and a few other places, and that makes me nervous.  Optimal has a particular meaning, so if you haven't proved something optimal, you're likely to get called out by a reviewer.  For anything you can't prove is optimal, I'd find a synonym.  "carefully tuned", "effective", "highly optimized"...}
% addressed

As a result, \frameworkName~achieves three key advantages over coarse-grained approaches:



\begin{enumerate}
    \item \textit{In-situ} Calibration: By leveraging code deformation for qubit isolation, QECali eliminates the need for logical SWAP operations, avoiding the substantial overhead associated with quantum state transfer and ancillary qubit preparation.
    \item Uninterrupted Computation:  Combining physical-level qubit isolation and dynamic compensation enables continuous logical operations during calibration, effectively eliminating computational stalls while maintaining error protection.
    \item Fine-grained Resource Management:  QECali's ability to isolate and calibrate individual physical qubits enables optimal resource utilization, allowing calibration schedules to be tailored to individual qubit drift patterns and error rates. 
\end{enumerate}

\begin{comment}
    The key insight to enable the advantages above is that --- since logical information is collectively encoded in a lattice patch, if we just separate out individual physical qubits for calibration, the logical computation can continue without stalling and being swapped out.


By creatively employing the \emph{code deformation} technique~\cite{yin2024surf, vuillot2019code, bombin2009quantum}, we can selectively isolate the qubits needing calibration without disrupting the quantum information encoded in the logical qubit. Once calibration is complete, the calibrated qubits are reintegrated into the system in an information-preserving manner. \frameworkName~achieves three key advantages that effectively resolve the primary limitations of the \policyTwoName~approach:


While enabling concurrent calibration and computation and significantly suppress space-time overhead, the isolated qubits reduce the redundancy in logical qubits and may degrade the QEC protection level. To address this, we leverage \emph{code enlargement}~\cite{vuillot2019code, suzuki2022q3de, yin2024surf} during calibration to restore the QEC protection level impacted by the isolation of qubits, preserving QEC capability while introducing only a modest qubit overhead.

\end{comment}

Our evaluation on both quantum hardware and simulation demonstrates QECali's effectiveness across different architectures and use cases. On practical quantum benchmarks such as quantum chemistry applications, QECali maintains sub-threshold error rates with only 12-15\% additional physical qubits and negligible impact on execution time, reducing retry risk by up to 85\% compared to baselines. Component-wise analysis shows that QECali's adaptive scheduling achieves 91\% reduction in calibration operations while minimizing space-time overhead. Our experiments on Rigetti and IBM processors validate QECali's key insight, showing that code deformation can effectively control error propagation.

In summary, this paper makes the following contributions:

\begin{itemize}

\item We introduce a novel framework,~\frameworkName, for concurrent calibration and computation in surface codes that leverages the collective nature of logical encoding to enable fine-grained physical qubit calibration without logical state transfer.

\item We design and formalize a novel instruction set based on code deformation for calibration in surface codes of grid and heavy-hexagon topology. This instruction set provides primitive operations for selective qubit isolation and patch compensation, enabling fine-grained control over code structure while preserving error correcting capabilities.

\item We develop an adaptive scheduling method that coordinates calibration operations across physical qubits while balancing multiple competing constraints: calibration parallelism, code distance preservation, qubit drift patterns, and hardware topology, achieving efficient, fine-grained calibration.

\item We introduce a set of key device metrics for characterizing quantum hardware, including calibration times, drift rates, and crosstalk. These metrics provide essential information for optimizing calibration schedules and predicting performance.

% For large-scale programs, it achieves a fidelity enhancement by several orders of magnitude over Enola. Additionally, it enhances the execution time of compiled programs by a factor of 1.71x to 3.46x, alongside a reduction of compilation time by approximately up to 213.5x.
\end{itemize}
% \dean{This is not really the place to summarize results ("contributions" should be more about ideas).  Summarize the results at end of intro, right before "contributions" (there's already
% a placeholder there).}
% \dean{Third one is kind of weak.  What's the novel idea there?}
\begin{comment}
    
\todoFX{(a) The qubit and links on the device have different qualities, lead to different fidelity of gates, which need to be calibrated differently in order to reach a uniform error rate. (b) Crosstalk and dependence between calibrations. Calibration of one gate may affect the quantum state on the nearby qubits.
[ref: Physical qubit calibration on a directed acyclic graph], Calibration cnot(q1, q2) need to calibrate single-Q gate on q1 and q2 first. (c) Trade off between calibration time and loss of code distance. If we isolate more qubit simultaneously, we can get a faster calibration, however this will lead to a higher distance loss (a) The qubit and links on the device have different qualities, lead to different fidelity of gates, which need to be calibrated differently in order to reach a uniform error rate. (b) Crosstalk and dependence between calibrations. Calibration of one gate may affect the quantum state on the nearby qubits.
[ref: Physical qubit calibration on a directed acyclic graph], Calibration cnot(q1, q2) need to calibrate single-Q gate on q1 and q2 first. (c) Trade off between calibration time and loss of code distance. If we isolate more qubit simultaneously, we can get a faster calibration, however this will lead to a higher distance loss }
\end{comment}




% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.47\textwidth]{Figures/motivation.png}
% \label{fig: Challege}
% \caption{(a) The qubit and links on the device have different qualities, lead to different fidelity of gates, which need to be calibrated differently in order to reach a uniform error rate. (b) Crosstalk and dependence between calibrations. Calibration of one gate may affect the quantum state on the nearby qubits.
% [ref: Physical qubit calibration on a directed acyclic graph], Calibration cnot(q1, q2) need to calibrate single-Q gate on q1 and q2 first. (c) Trade off between calibration time and loss of code distance. If we isolate more qubit simultaneously, we can get a faster calibration, however this will lead to a higher distance loss 
% }
% \end{figure}

% qubits in the same code patch require different calibration periods due to their heterogeneous qualities, but this



% Scheduling, take the prior information of hardware conditions into consideration, pre-determine a calibration strategy during runtime

% This brings us to our proposed solution. Current calibration approaches do not fully account for the heterogeneous quality of individual qubits. In this paper, we propose a hardware-aware fine-grained calibration method that isolates specific gates and qubits using code deformation techniques from the surface code. By selectively performing destructive calibration on lower-quality qubits and gates, we can enhance overall efficiency without significantly affecting the logical error rate.


% We design calibration schedule based on hardware information (hardware-aware)

% Preemptively choose a larger distance to keep the QEC capability during calibration; trade-off: more distance reduction, less calibration time, because more qubits can be calibrated simultaneously

% software solution for hardware problem for free with negligible time overhead


% \YS{These naive approaches highlight the inherent challenges of maintaining error correction without real-time calibration. The only way to ensure consistent error suppression over long runtimes is to integrate calibration directly into the QEC process, allowing for continuous adjustment of control parameters in response to error drift. However, performing calibration concurrently with QEC presents significant challenges, particularly due to the need to maintain logical qubit coherence without disrupting the error correction cycle. This necessitates a sophisticated strategy to synchronize calibration with QEC operations, ensuring that both processes can run in tandem without compromising the logical state of the quantum computation. The critical question becomes: \textbf{How can we achieve efficient calibration during runtime while preserving the integrity of the QEC cycle?}}

% \YS{To address this question, preliminary approaches have been explored, aiming to enable calibration without compromising the QEC process. One such approach, described in [4], attempts to calibrate based on detection events. This statistical approach updates control parameters using error rates inferred from error syndromes without interrupting error detection. However, this method faces significant limitations: inaccuracies in inferring control parameters from syndromes and complications arising from the degeneracy of QEC codes. Degeneracy—where different physical errors produce identical error syndromes—makes it difficult to accurately identify the faulty qubit, thereby reducing the effectiveness of this approach.}

% We believe that the best solution lies in having QEC and calibration run in tandem. This raises important questions around timescales: How long does calibration take? How does it interact with the QEC cycle? Since QEC requires continuous operation to preserve logical states, it cannot simply be paused for calibration. The challenge, then, is how to balance these two processes.
% \todoFX{Challenge of integrating QEC and calibration. In order for them to happen simultaneously, (1) Need to be in-situ. Moving logical qubits induce large overhead, (2) Need to be fine-grained. The calibration on targeting qubits should not affect the operations on other qubits. (3) Complexity in Scheduling: heterogeneous qubits, different qubits have different quality, need different time duration for each qubit's calibration; dependence in gate calibration, may need to disable adjacent qubits}




==> TexFile/03_background_01.tex <==
\section{Background}
\label{sec:background}
In this section, we first provide an overview of the FTQC architecture based on surface codes, along with background information on error drift and calibration. We then introduce the code deformation framework, \emph{Surf-Deformer}~\cite{yin2024surf}, which serves as the foundation for the qubit isolation and code enlargement operations in our solution.

\subsection{FTQC Based on Surface Code}{\label{subsec: surface code}}
\noindent\textbf{Surface code basics. }Surface code is the leading candidate for realizing FTQC due to its simple 2D grid structure and its high error threshold ($\sim 1\%$) compared to others \cite{bravyi1998quantum, fowler2012surface}. The key ingredients of surface codes are as follows.

\emph{Data and syndrome qubits}. A surface code patch encodes multiple physical qubits as a single \emph{logical qubit}, as shown in \cref{fig}(a). The physical qubits in the code have two types: \emph{data qubits} (black dots) and \emph{syndrome qubits} (white dots). Data qubits store the logical quantum state, while syndrome qubits collect error information on their adjacent data qubits.

\emph{Stabilizers.} Each syndrome qubit is associated with a \emph{stabilizer} \cite{gottesman1996class, gottesman1998heisenberg, nielsen2010quantum}, a Pauli operator involving the adjacent data qubits. These stabilizers can involve four data qubits (squares), or two data qubits (half circles). The syndrome qubits indicate the measurement outcomes of these stabilizers, yielding \emph{error syndromes} that help to deduce potential error corrections. 

\emph{Logical operation. } A \emph{logical operation} takes a legitimate logical state to another, and cannot be detected as an error through stabilizer measurements. Notably, a logical operation should commute with all stabilizers but is not a product of stabilizers. An $X$ (resp. $Z$) logical operation is denoted by a red (resp. blue) line in Figure \ref{fig SurCodeEx}, consisting of the product of $X$ (resp. $Z$) Pauli operators on the data qubits on the line. 

\emph{Code distance. }The \emph{distance} of a code is defined as the minimal number of qubits contained in a logical operation. In the case of a perfect standard surface code, the code distance is equal to the number of data qubits on its edge. Figure \ref{fig SurCodeEx}(a) gives an example of a surface code of distance $5$. Code distance indicates the QEC capability because the logical error rate decays exponentially in code distance, as long as the physical error rate remains below a certain threshold. For a more in-depth discussion, please refer to \cite{fowler2012surface, dennis2002topological}.

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.20]{figures/Surface Code.pdf}
% \caption{A perfect surface code with code distance $5$.}
% \label{fig SurCodeEx}
% \end{figure}

\subsection{Error Drift and Calibration}

\subsection{Error Drift}
error drift~\cite{ravi2023navigating, burnett2019decoherence}
TLS~\cite{martinis2005decoherence}

heterogeneous quality, distinct calibration period
\emph{Destructive Calibration. }
Qubit calibration, gate calibration

\subsection{Surf-Deformer}

\cite{yin2024surf} develops a framework that dynamically detect defected qubits and remove them by code deformation, while enlarging the code patch to recover the code distance. In this paper, we borrow this idea to isolate the qubits to be calibrated from the system.


construct new stabilizers that do not involve the defect

\noindent\textbf{Qubit Isolation via Code Deformation.}

\noindent\textbf{Distance Loss and Code Enlargement}

Emphasize that it does not affect the on-going computation.


% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.30]{figures/proposal.pdf}
% \caption{
% Motivational Example: (a)A d=5 Surface Code, defective qubits are denoted by a red "X," and the logical X operator is enclosed by a red dashed line. (b) A code can operate on the defective coupling graph, but the logical X from (a) serving as the stabilizer. (c) A deformed code that shares the logical X from (a) and can undergo deformation through direct measurements of the stabilizers.
% }
% \label{fig:motivation example}
% \end{figure}



% \begin{figure}[h]
% \centering
% % \includegraphics[scale=0.20]{figures/calibration.pdf}
% \label{fig SurCodeEx}
% \end{figure}

==> TexFile/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip

